On Intrinsic Dataset Properties for Adversarial Machine Learning

Deep neural networks (DNNs) have played a key role in a wide range of machine learning applications. However, DNN classifiers are vulnerable to human-imperceptible adversarial perturbations, which can cause them to misclassify inputs with high confidence. Thus, creating robust DNNs which can defend against malicious examples is critical in applications where security plays a major role. In this paper, we study the effect of intrinsic dataset properties on the performance of adversarial attack and defense methods, testing on five popular image classification datasets - MNIST, Fashion-MNIST, CIFAR10/CIFAR100, and ImageNet. We find that input size and image contrast play key roles in attack and defense success. Our discoveries highlight that dataset design and data preprocessing steps are important to boost the adversarial robustness of DNNs. To our best knowledge, this is the first comprehensive work that studies the effect of intrinsic dataset properties on adversarial machine learning.

==> doc/algo.tex <==
\section{Methodology}
\label{sec:algo}

In this section, we present our RAQ methodology. Our approach consists of two algorithms 

RAQ-LD and RAQ-RL


\subsection{RAQ with Linear Decision Block (RAQ-LD)}



\textcolor{red}{Will add a figure to illustrate the flow}

A simple approach to runtime activation quantization is a heuristic based method. In such a method, we can consider the input feature map for each layer we wish to quantize. We can pass the input feature at each layer through an auxiliary network that converts the feature map into a fixed embedding. Based on such a fixed embedding, we can decide what bitwidth to use for the corresponding layer via a simple decision network. The objective of this heuristic method is to decide the bitwidth for each layer by training a simple linear decision network on the input feature map of the given layer. We implement such a method by adding a small side network to each convolutional layer \( \mathcal{C} \) we wish to quantize. This side network consists of a fully-connected layer that encodes the input channels of \( \mathcal{C} \) to a hidden dimension size. We can pass this hidden embedding through another fully-connected layer and sigmoid layer to arrive at a single float action. We use such a continuous action \textit{a} to determine the bitwidth as done by \red{insert reference to HAQ}:

\begin{align}
&\text{round}(b_{min} - 0.5 + \alpha_{k} \times (b_{max} - b_{min} + 1)), 
\end{align}

Such side networks can be easily inserted into existing architectures. Once RAQ-LD side networks are inserted into a pretrained model architecture, we can fine-tune the weights of the side networks by retraining our network. 

\subsection{RAQ with Reinforcement Learning (RAQ-RL)}

\textcolor{red}{Will delete the following, but maybe use some math notations...}

\textcolor{red}{Will add a figure to illustrate the flow}

Figure~\ref{fig:framework} shows the overall flow of our RAQ-RL flow. It optimizes layer-wise bitwidths.
The trained hyper-parameters are XXX.


Our training objective can be written as follows,

The controller is trained to 

Environment

Agent

\begin{figure}[t]
\centering 
\includegraphics[width=0.45\textwidth]{./figs/RAQ-RL-model.pdf}
\caption{
Illustration of our RAQ-RL framework.
}
\label{fig:framework} 
\end{figure}


% Note that update \eqref{eq:e_meta_grad} involves a gradient through a gradient. 
% Computationally, this requires an additional backward pass through 


\begin{algorithm*}[ht]
\begin{algorithmic}[1]
% \State \textbf{Goal}: Search neural architecture $a$ along with layer-wise bitwidths $b$. 
\Repeat
\State Sample minibatch of network configurations $\{\alpha_i\}_{i=1}^{k}$ from the controller $\pi_\theta$
\State Update network models $\{w(\alpha_i)\}$ by minimizing the training loss following Eqn. \ref{eq:approx_w}.
% \State Update $a, b$ by descending on validation set following Eq.~\ref{eq:meta_update}.
\State Update the controller parameters $\theta$ following Eqn.~\eqref{eq:meta_update} and \eqref{eq:reinforce}.
\Until{Converge}
% \State \textbf{Output}: $a, b$.
\end{algorithmic}
% \caption{Proposed Algorithm}\label{alg}
\caption{Energy aware neural architecture search} \label{alg}
\end{algorithm*}

%% explain the algorithm here
% In Algorithm \ref{alg}, 


\begin{figure*}[ht]
\centering 
\includegraphics[width=0.98\textwidth]{./figs/nas.png}
\caption{
An illustration of the structure of a MB search unit.
$m$ denotes the expand ratio,
$k$ denotes the kernel size,
$s$ denotes whether skipping this block,
and $b_1$, $b_2$ denotes the layer-wise bitwidths.
% If the expand ratio not equals to 1, one block contains three convolution layers.
% The first is the expanded layer (pointwise), the second is the depthwise layer, and the third is a pointwise layer.
}
\label{fig:mbconv} 
\end{figure*}


\subsection{Search Algorithm}
We are now ready to show the representation of 
the network configuration $\alpha$.
% \red{need a figure here...}
Let $\eta_\ell = [s^{\ell}, m^{\ell}, k^{\ell}, b_1^{\ell}, b_2^{\ell}]$ 
be the discrete variables that
associated with the MB block in the $\ell$-th layer.
% Denote a 
% Denote $B1, B2$ as the set of $b_1^{\ell}, b_2^{\ell}$, respectively.
% Denote $\{a_i=[o_1, \cdots, o_N]^i \in \R^{5\times N}\}_{i}$ 
% as neural network configuration samples drawn from $\pi_\theta(\alpha)$.
A network configuration $\alpha$ is a stack of $N$ MB
blocks as a vector of
$[\eta_1, ..., \eta_N] \in \R^{5N}$, where $N$ 
denotes the number of MB blocks.
Each element in $\alpha$ can be considered as a specific operation.
Without loss of generality,
denote $o(x)$ as one of the operator defined in $\alpha$, 
which takes $K$ possible values.
E.g., $o(x)$ could be a depthwise convolution layer, 
% with filter size $k\times k$, 
in this case, all possible filter size choices are $\{3\times3, 5\times5, 7\times 7\}$ and $K=3$.
Given the input $x$, $o(x)$ maps $x$ to its corresponding output.

To learn the controller, it remains to show the representation of $\pi_\theta$ 
and the gradient of the validation loss $\nabla_\theta \E_{\alpha\sim \pi_\theta}[\loss(f_{w'}(\alpha),\D^{val})]$ w.r.t. $\theta$ defined in Eqn. \ref{eq:meta_update}.
For each operator $o(x)$, 
we represent discrete valued architecture choices
as a one-hot vector $d\in \R^K$, 
such that $d_j\in \{0,1\}$ and $\sum_{j=1}^K d_j=1$.
In this way, the corresponding output of applying operator $o$ with representation $d$ is
$\sum_{j=1}^K d_j o_j(x)$, where $o_j(x)$ denotes the forward operation with $j$-th candidate in the search space (e.g., $o_1$ could be $3\times 3$ depthwise convolution).
% We restrict ourselves to a representation of a one-hot vector $d\in \R^K$,
% namely, $d_j \in \{0, 1\}$ and $\sum_{j=1}^K d_j=1$ for discrete valued samples.
% vector of binary bits ($\{0,1\}$) 
% that are one-hot,
% For each operator, 
We parametrize $p(d_j = 1) = {\exp(\phi_j)}/{\sum_{i=1}^K \exp(\phi_i)},$
where  $\{\phi_j\}$ are trainable parameters that belongs to the controller parameters $\theta$.
It is problematic to calculate the gradients directly 
due to the inability to back-propagate through categorical samples.
We thus replace the non-differentiable network configuration samples with
continuous differentiable samples from a Gumbel-Softmax
distribution \citep{gumbel_softmax}.
That is, we replace one-hot representation $d$ as a continuous vector
such that $d_j \geq 0, \sum_{j=1}^K d_j=1$, 
which can be trained using standard back-propagation.
For the rest,
we follow the settings for Gumbel-softmax sampling used
in FBNet \citep{wu2018fbnet}.

% \red{I am trying to hide all Gumbel-Softmax and differentiable NAS details since it is not our main contribution. Not sure whether the method part itself is clear enough..}

% % It is obvious the loss function in Eq.~\ref{eq:loss_main} is not directly differentiable to the sampled discrete variable $a$.
% % Therefore, we relax the discrete variable to a Gumbel-Softmax over all possible choices:
% % \begin{equation}
% % \label{eq:operation}
% %     x_{out} = \sum_{k=1}^{K}{p_k o_k(x_{in}, w_k)},
% % \end{equation}
% \begin{equation}
% \label{eq:gumbel-softmax}
% p(s^{\ell} = 0) = \frac{\exp{((\log{z_0} + G_0) / \tau)}}{\sum_{i \in \{0, 1\}}{\exp{((\log{z_i} + G_i) / \tau)}}},
% \end{equation}
% where $\{G_i | i \in \{0, 1\} \}$ is a sequence of standard Gumbel random variable,
% and can be sampled from a standard Gumbel distribution $G = - \log (- \log (X))$
% with a uniform distribution $X \sim [0, 1]$.
% $\tau$ is the temperature.
% Smaller $\tau$ forces $p_k$ to be more similar to a discrete variable.
% This process is described in Figure~\ref{fig:gumbel}. 
% During the feed forward period,
% one certain layer is sampled from all the choices 
% and the gradient is passed through during the back propagation.

% \paragraph{Mixed precision}
% In addition, we allow each layer to adopt precision (bit-width) adaptively. 
% Specifically, 
% let $\{b_i\}_{i=1}^N$ be a set of candidiate precision bits, 
% % We change the forward calculation in Eq.~\ref{eq:operation} to:

% \begin{equation}
% \label{eq:mixed}
%     x_{out} = \sum_{i=1}^{N}[p_i \sum_{k=1}^{K}{p_k o_k^{n}(x^{n}_{in}, w_k, b_i)}]
% \end{equation}
% where $o_k^{n}$ denotes the operation $o_k$ is quantized to $n$ bits, $x^{n}_{in}$ denotes the input $x_{in}$ is quantized to $n$ bits.
% In practice, 
% we constrain the weight and input for each layer have same bits 
% to reduce the search space and therefore save search time.

% \begin{figure}[h]
% \centering 
% \includegraphics[width=0.38\textwidth]{./figs/gumbel_softmax.png} \\
% \caption{This figure shows how Gumbel-Softmax works.
% This estimator samples a discrete variable during feed forward,
% and obtain an gradient by re-parametric trick. 
% \red{use some histogram figure to represent the policy distribution?}}
% \label{fig:gumbel} 
% \end{figure}

% Notice that our search unit is MBConv blocks, 
% which each contains two or three convolution layers.
% Shown in Figure~\ref{fig:mbconv},
% some parts of the convolution layer are depthwise convolution layers,
% while others are pointwise convolution layers.
% depthwise convolution layer contains more parameters, which could exhaust more energy.
% Therefore, in practice, we assign two different bitwidths for one MBConv block,
% one is for the pointwise layers and
% the other is for the depthwise layer.
% As shown in Figure~\ref{fig:mbconv}, the bit-width for pointwise layers is defined as $b_1$ and the other is defined as $b_2$.
% Then, the forward process described in Eq.~\ref{eq:mixed} is converted to:
% $$
% x' = \sum_{i=1}^{N}[p_{1i} \sum_{k=1}^{K}{p_k o_k^{n}(x^{n}_{in}, w_k, b_{1i})}],
% $$
% $$
% x' = \sum_{i=1}^{N}[p_{2i} \sum_{k=1}^{K}{p_k o_k^{n}(x'^{n}, w_k, b_{2i})}],
% $$
% $$
% x_{out} = \sum_{i=1}^{N}[p_{1i} \sum_{k=1}^{K}{p_k o_k^{n}(x'^{n}, w_k, b_{1i})}].
% $$
% \subsection{Training with Quantization}
% Recent works~\cite{wang2018haq, wu2018mixed} search layer-wise bitwidths for a pre-trained model.
% Consequently, these works avoid the problem of training a network with low precision.

% We, however, motivate to search neural architecture with mixed bitwidths
% and only quantize a trained model will break the joint search space.
% Therefore, we propose to quantize the neural network during training.
\textbf{Training with Quantized Weights.}
In our approach, only the quantized values of the weights and activations are used in all forward operations.  
% During the training stage, we still use full precision gradients.
In order to learn quantized weights,
we follow the linear quantization schemes suggested by \cite{wang2018haq, ren2018admmnn}. 
Specifically, for a layer with $n\times d$ dimensional input $\pmb{x}  =(x_1, ..., x_n), x_i\in \R^d$, 
we quantize each $x_i$ linearly into $b$ bits:
$$
\mathrm{Quantize}(x_i, b) = \mathrm{round}(\mathrm{clamp}(x_i, c) / s) \times s,
$$
where $\mathrm{clamp}$ truncates all values into the range of $[-c, c]$, with  $c=\max\{|x_i|\}$. And the scaling factor $s$ is defined as
$s=c / (2^{b-1} - 1)$.

% % For each iteration, we calculate weight for $o_k^{n}$ as:
% $$
% w_k^{*} = \mathrm{Quantize}(w_k),
% $$
% $$
% x_{out} = \sum_{n=1}^{N}[p_n \sum_{k=1}^{K}{p_k o_k^{n}(x^{n}_{in}, w_k^{*})}],
% $$
% where $\mathrm{Quantize}$ is a differentiable function,
% and thus the gradient can be passed to $w_k$.
% In practice, 
% we first layer-wise truncate $w_k$ into the layer-wise range of $[−c, c]$, 
% and we then quantize it linearly into $n$ bits.
% $$
% \mathrm{Quantize}(w_k, n ,c) = \mathrm{round}(\mathrm{clamp}(w_k, c) / s) \times s,
% $$
% where $\mathrm{clamp}(\cdot, c)$ is to truncate the values into $[−c, c]$, 
% and the scaling factor $s$ is defined as
% $$
% s=c / (2^{n-1} - 1).
% $$
% In practice, we find that $c=\max\{|w_k|\}$ works well for all the cases.
% out that setting $ c = \max{|w_k|} $
% or setting 
% $$
% c = \mathrm{argmin}_{x}KL(w_k || \mathrm{Quantize}(w_k,n,x))
% $$ 
% both work. 
% We adopt the strategy $c = \max{|w_k|}$ to save time,
% since calculating $c = \mathrm{argmin}_{x}KL(w_k || \mathrm{Quantize}(w_k,n,x))$ layer-wise for each iteration is expensive.

% \subsection{Summary}

% In this work, 
% we construct a layer-wise search space with a fixed macro-architecture. 
% Each layer can choose a different layer and two different bitwidths,
% one is for the depthwise layer, and the other is for the pointwise layer.
% The search space is summarized in Table~\ref{table:search-space}.
% % The available bitwidths is $\{2, 4, 6, 8\}$.
% We have defined the upper bound of the number of layers and the input/output dimensions of each block.
% We also pre-define the layer type and bitwidth for the first and last two layers.

% % We then use differentiable neural architecture search the neural architecture and adaptive bitwidths.
% % Our algorithm is summarized in Algorithm~\ref{alg}.




==> doc/old/defense.tex <==
\section{Adversarial Defense Strategies}
\label{sec:defense}

In this section, we will cover adversarial defense strategies by their three main categories — input transformation and compression, adversarial retraining, and intrinsic state modeling. For each section, we will cover specific defense techniques and their advantages and drawbacks.

\subsection{Input Transformation and Compression}
\label{defense:transform}

Several works have explored the use of input transformations and compression techniques to try to reduce the impact of adversarial perturbations. Dziugaite et al.\cite{dziugaite2016study} explored the use of JPEG compression to smooth input images before model inference, discovering that JPEG compression is effective in some cases in reducing the drop in classification accuracy for small perturbation sizes. Additionally, Guo et al. \cite{guo2017countering} attempted using total variance minimization \cite{rudintvm} and other image transformations to counter adversarial perturbations, discovering that total variance minimization can significantly improve the robustness of DNNs to adversarial attack.

\subsection{Adversarial Retraining}
\label{defense:retraining}

The second defense strategy lies in adversarial retraining, where a model is retrained on adversarially-generated inputs to improve its robustness. However, Tramèr et al. \cite{tramr2017ensemble} discovered that naïve adversarial training often fails to defend against adversarial perturbations as the model learns to generate weak perturbations rather than learning to defend against strong attacks. They introduced ensemble adversarial training, which augments a model's training data with perturbations transferred from other models. Ensemble adversarial training creates models that are significantly more robust to adversarial attacks.

==> doc/old/evasion.tex <==
\section{Adversarial Attacks}
\label{sec:evasion}

In this section, we introduce a selection of commonly used adversarial attacks and their methodologies.

\subsection{Fast Gradient Sign Method (FGSM)}
\label{evasion:fgsm}

Goodfellow et al. \cite{goodfellow2014explaining} introduced the Fast Gradient Sign Method (FGSM), which quickly takes the gradient of the cost function with respect to a given input. For a cost function $J$ of a model with parameters $\theta$, input $x$, and label $y$, FGSM linearizes the cost function at the current $\theta$ and generate adversarial examples using the following optimization algorithm:

$$\rho = \epsilon \cdot \text{sign}(\nabla_x J(\theta, x, y))$$

As a simple gradient calculation that can be computed quickly through backpropagation, FGSM provides a cost-effective method to adversarially perturb an input to a neural network.

\subsection{Projected Gradient Descent (PGD)}
\label{evasion:pgd}

Projected Gradient Descent (PGD) is a first-order attack method introduced by Madry et al. \cite{aleks2017deep} PGD is a multi-step, iterative gradient-based attack that attempts to maximize the loss function via the following equation:

$$x^{t+1} = \Pi_{x+S}(x^t + \epsilon \cdot \text{sign}(\nabla_x J(\theta, x, y))$$

Essentially, one can view PGD as a multi-step variant of FGSM. The additional attack effectiveness from multiple iterations makes PGD a powerful first-order adversary.

\subsection{DeepFool}
\label{evasion:deepfool}

DeepFool \cite{moosavidezfooli2015deepfool} attempts to calculate adversarial perturbations by perturbing a given input $x_0$ along the orthogonal projection of $x_0$ to its separating decision boundary. At each iteration, DeepFool linearizes the model function $f$ at the current point $x_i$ and then computes a minimal perturbation as:

$$\underset{r_i}{\text{argmax}} {||r_i||}_2 \text{ subject to }  f(x_i) + \nabla f(x_i)^{T}r_i = 0.$$

\subsection{Carlini-Wagner (CW)}

The family of Carlini-Wagner (CW) attacks \cite{carliniwagner} starts with Szegedy et al.'s formulation of the adversarial example problem as a constrained minimization problem \cite{szegedy2013intriguing}:

\begin{align*}
\text{minimize } &\mathcal{D}(x, x+\delta) \\
\text{such that } &{C}(x+\delta) = t \\
& x + \delta \in [0, 1]^n \\
\end{align*}

\noindent where $\mathcal{D}$ is some distance metric (one of $L_0, L_2, L_{\infty}$), $C$ is the targeted classifier, $t$ is the target label, and $\delta$ is the perturbation. We wish to minimize $\delta$ such that the perturbed image remains similar to the original image, yet is still misclassified. As the above optimization problem is difficult to solve, Carlini et al. rewrite it as the following:

\begin{align*}
& \text{minimize } \mathcal{D}(x, x+\delta) + c \cdot f(x+\delta) \\
& \text{such that } x + \delta \in [0, 1]^n
\end{align*}

\noindent where $f$ is an objective function such that $C(x+\delta) = t$ if and only if $f(x+\delta) \leq 0$ and $c$ is some constant $> 0$. This formulation allows for gradient descent to easily solve the optimization problem. The Carlini-Wagner attacks are very powerful, with higher attack success rates than other methods.  

\subsection{Basic Iterative Method (BIM)}

An extension of FGSM, the Basic Iterative Method (BIM) applies FGSM multiple times with a small step size, clipping pixel values after each step to ensure that the perturbed image remains within the $\epsilon$-neighborhood of the original image. Formally, the perturbed image is defined as:

$$x_0^{adv} = x, x_{N+1}^{adv} = Clip_{x, \epsilon}\{x_N^{adv} + \alpha \text{sign}(\nabla_x J(\theta, x_N^{adv}, y)\}.$$

==> doc/old/results.tex <==
\section{Discussion and Future Research}
\label{sec:results}

{\red{Move this section's results/observations to the Experimental Results section. Move the future research part to conclusion.}

Our experimental results suggest several intriguing conclusions concerning adversarial machine learning techniques.

\textbf{Intrinsic Dataset Attributes}

{\red{X-rays and GTSRB are additonal results that you can show in the experimental results?}

The varying performance of the attack and defense methods we tested across datasets highlights how dataset properties can drastically affect the performance of adversarial machine learning techniques. For instance, image compression defenses worked significantly better on the Chest X-rays dataset than on GTSRB. One explanation for this discrepancy may lie in the input image size. While Chest X-rays consists of higher-quality images reshaped to $224 \times 224$, GTSRB images are significantly smaller, with a size of only $32 \times 32$. GTSRB images inherently have less input features than Chest X-ray images. On Chest X-rays, image compression defenses successfully remove adversarial perturbations while leaving enough useful features for successful classification. However, on smaller GTSRB images, compression defenses may inadvertently remove too many features along with adversarial perturbations.

Additionally, we spent significantly more time tuning our attacks and defenses on GTSRB than on the Chest X-rays dataset. We suggest that this additional hyperparameter tuning time also stems from the nature of the different datasets. Although GTSRB consists of smaller images than Chest X-rays, GTSRB has significantly more images (50,000+ compared to 5,863). Thus, our GTSRB model successfully learned to classify noisy, low-resolution images with great accuracy. As a result, our original model already started off with some inherent robustness to noisy perturbations. However, once we tuned a successful GTSRB attack, the attack became very difficult to defend against because of the small input sizes of GTSRB images.

We believe that effect of intrinsic dataset properties on adversarial performance is a promising future research direction which may inform new adversarial defense strategies.

\textbf{Modeling Defenses}

Across various datasets and attack methods, the I-defender modeling defense consistently led to good defense results comparable to other defense methods. While other defense methods required some parameter tuning to achieve good results, I-defender worked effectively without any tweaking. Thus, we hope that future research will continue exploring the potential of modeling defenses as a general defense against adversarial attacks, providing a more concrete guarantee of robustness.
